Strategizing EV Charging and Renewable Integration in Texas

Exploring the convergence of electric vehicles (EVs), renewable energy, and smart grid technologies in the context of Texas, this study addresses challenges hindering the widespread adoption of EVs. Acknowledging their environmental benefits, the research focuses on grid stability concerns, uncoordinated charging patterns, and the complicated relationship between EVs and renewable energy sources. Dynamic time warping (DTW) clustering and k-means clustering methodologies categorize days based on total load and net load, offering nuanced insights into daily electricity consumption and renewable energy generation patterns. By establishing optimal charging and vehicle-to-grid (V2G) windows tailored to specific load characteristics, the study provides a sophisticated methodology for strategic decision-making in energy consumption and renewable integration. The findings contribute to the ongoing discourse on achieving a sustainable and resilient energy future through the seamless integration of EVs into smart grids.

==> EE-Pockets.tex <==
Energy flexibility is the ability of energy producers or consumers to adjust their output power (generation by producers) or their energy consumption level (demand of consumers, e.g. shifting or reducing loads) \cite{junker2018characterizing}. Energy flexibility comes in many forms and presents itself in bulk power grids as well as microgrids and urban electric systems \cite{ThornburgACM}. In residential buildings, for example, energy flexibility is available when homeowners are willing for their home AC units to have shifting temperature setpoints that respond to load reduction request from the grid manager. Certain strained electrical utilities send out these requests in peak demand hours (e.g., 4-9PM in Southern California, when residential loads rises and solar power drops). Unless the grid takes direct control of the load in question, the energy flexibility is dependent on end-user cooperation. Another example of energy flexibility comes from regulating power output of a solar farm to help the grid operator stabilize the bulk power grid during extreme weather events. 

Utilizing energy flexibility from ERs is more challenging than leveraging flexibility of large consumers (e.g., industrial facilities) or utility-scale power producers (e.g. generation plants). The difficulty with DERs comes because individually they provide small pockets of flexibility but are constantly growing in number, geographical spread, and heterogeneity. If used effectively, distributed pockets of energy flexibility offered by DERs can be a reliable resource for grid management given their closer proximity to end-use facilities when compared to the grid manager (central) node. Furthermore, the distributed nature of DERs adds to the grid's flexibility for control across the network \cite{ThornburgKrogh2016}, \cite{Ustun2016}. Scalable aggregation is the key in unlocking the massive potential of DERs.

\vspace{-.15cm}
\subsection{Coordination Challenges}
\vspace{-.1cm}
IoT-connected DER controllers have a wide-range of communication and computation capabilities. This heterogeneity poses a challenge for utilizing federated computations to orchestrate DER functionalities. Put differently, data storage limitations, communication overhead, and computational constraints can degrade the performance of the analytics performed on local devices \cite{imteaj2020federated}. Moreover, the heterogeneity and multi-modality of the data collected by IoT-connected DERs pose additional difficulties in performing computations across these devices. Architectural design and computation process on edge IoT devices are extensively studied in the literature\cite{chen2019joint,chen2018federated,das2019privacy}. In what follows, we elaborate on key issues and discuss how they apply to the multi-agent DER context.

Agent hardware limitations, including constrained data storage and restricted computational and communication capabilities, can negatively affect cross-agent collaboration in multi-agent settings. These limitations slow down local computational process by increasing communication overhead and hindering intra-agent coordination. Hence, hardware specifications must be taken into account when implementing federated computations. For example, authors in \cite{hard2018federated} study hardware requirements for implementing next word prediction for a user typing. These hardware issues are even more visible in the context of nascent IoT-connected DERs.
The standards and requirements for the DER hardware setups are not yet well-defined. Manufactures and vendors are pursuing different communication protocols (e.g. OpenADR \cite{mcparland2011openadr}) while experimenting with computational possibilities. A gap also persists between access to device monitoring and measurement information in the same class of assets (e.g., solar PV inverters). 

Quality and frequency of information exchange among agents of a multi-agent network directly impact overall performance of the network. In multi-agent information processing setups, agents with limited communication resources can hinder convergence across the network. In addition, the trade-off between communication cost and frequency should be accounted for in designing federated computations \cite{ma2017distributed}. To address this issue, researchers have proposed a wide-range of solutions such as reducing the number of inter-agent information exchanges and reduce the size of exchanged message \cite{konevcny2016federated}. Accounting for communication limitations is more critical in the \gls{ders} energy management context since maintaining supply and demand balance is the key in preserving power grid's reliability. Wide-spread communication disruption can unbalance equity of generation and consumption and lead to power outages. Hence, developing robust federated computation methodologies for achieving energy management goals is critically important. 

The aforementioned issues (i.e., computation and communication constraints) leads to emergence of straggling agents. Stragglers fail to share or compute updates in time. Selective engagement of resourceful agents (computationally and communication-wise) could be a possible solution to address this issue \cite{das2019privacy}. Asynchronous implementation of updates \cite{mohammadi2015asynchronous} also alleviates this issue.
%Underutilized sources ...
Finally, depending on their location IoT-connected \gls{ders} might be governed by different policies. For example, some utilities allow \gls{ders} to provide a wide-range services for the grid while others may restrict participation to a specific aggregation arrangements. This heterogeneity of policies is an obstacle that limits coordination between DER agents located in different utility territories.

\vspace{-.2cm}
\subsection{Energy Management in DER Networks}
\vspace{-.1cm}
The following is a generic form of an optimization algorithm for operating a DER fleet. The algorithm is formulated so the optimum can be solved for in a centralized fashion \cite{mohammadi2020federated}. %The following equations formulate this problem as:

\vspace{-.1cm}
\small
\begin{subequations}\label{generalproblem}
\begin{align}
&\displaystyle \underset{{x}_{k}}{\text{minimize}}\;\; \sum_{k\in \Omega_{\text{agents}}} f_k(x_k)\label{main_obj}\\
&\text{s.t.}\hspace{1.04cm} g_j(x)\leq 0; \;\; (:\mu_j) \;\;\; j\in \Omega_{ineq} \label{ineq_cnst}\\
&\hspace{1.5cm} h_j(x)= 0;\;\;(:\lambda_j) \;\;\; j \in \Omega_{eq} \label{eq_cnst}
\end{align}
\end{subequations} 
\normalsize

In this setup the objective function ($f_k(\cdot)$) can capture a wide-range of goals including energy cost or emission minimization that $k$ agents (i.e., \gls{iot}-connected \gls{ders}) are collectively aiming to achieve. Also, sets of all agents, inequality constraints, and equality constraint are represented by $\Omega_{\text{agents}}$, $\Omega_{ineq}$, and $\Omega_{eq}$ , respectively. Moreover, $x_k$ denotes the variables associated with agent $k$. 
Inequality and equality constraints associated with each agent are denoted by  $g_j(\cdot)$ and $h_j(\cdot)$. Variables $\mu_j$ and $\lambda_j$ are Lagrangian multipliers associated with inequality and equality constraints, respectively.

Numerous solution approaches exist that are based on finding a solution that satisfies the first-order optimality conditions of this problem. % \cite{Mohammadi2016}. 
These conditions can be derived from the Lagrangian function of original optimization problem \eqref{generalproblem}. Henceforth these conditions will be denoted by $\mathfrak{O}$.

\vspace{-.2cm}
\subsection{Inter-Agent Analytics}
\vspace{-.1cm}
To directly solve the first order optimality conditions of the underlying optimization problem of \eqref{generalproblem} above, a novel federated computation framework is needed. Thus, technically reduces the optimization problem to finding a solution for a coupled system of equations with geometric constraints. This system of equations can be solved in a fully distributed manner through an iterative process. This is due to the fact each equation only contains local variables (i.e., related an agent or its neighboring agents)


This iterative process relies on the agents to conduct local updates and information exchange. In the case that a problem formulation includes constraints of the physical power network, physical-connections needs to be reflected in the communication graph. Each agent $i$ is only required to update variables associated with itself (namely $V_{i}$) and share updates with a limited number of other agents. Collectively, agents of this multi-agent system solve the optimality conditions of the underlying optimization problem. In order to solve the discussed set of equation, the federated computation framework creates local copies of shared variables and assign each copy to a corresponding agent \cite{olfati2007consensus}. %,olfati2005consensus}. 
The iterative process ensures that all the local copies converge to the same value. The formula for local updates of each agent is presented below, where the consensus term enforces agreement between local copies of agents. The final term uses the updated copies to solve the optimality conditions.

\vspace{-.2cm}
\small
 \begin{eqnarray}
V_{i}(k+1)&=&\mathbb{P}[V_i(k)+{\boldmath\rho}_i^\mathcal{C}(k) \overbrace{\sum_{j\in\Omega_i}(V_i(k)-V_j(k))}^{\text{neighborhood consensus}}\label{y_update}\\  \nonumber && +{\boldmath\rho}_i^\mathcal{I}(k) \underbrace{\mathfrak{O}_i(V_i(k))}_{\text{optimality conditions}}]_\mathcal{F}, \; \; j\in \Omega_i
  \end{eqnarray}
\normalsize

% \begin{equation}
% V_{i}(k+1)=\mathbb{P}[V_i(k)+{\boldmath\rho}_i^C \sum_{j\in\Omega_i}(V_i(k)-V_j(k))+ 
% {\boldmath\rho}_i^I \mathfrak{O}(V_j(k))]_\mathcal{F}, \; \; j\in \Omega_i
%   \label{y_update}
%   \end{equation}

In \eqref{y_update}, $V_{i}$ is the collection of variables associate with agent $i$ including $x_i,\mu_j, \lambda_j$. Also, $k$ denotes the iteration number whereas $\Omega_i$ represents the neighboring set of agent $i$. 
Furthermore, $\mathfrak{O}_i(\cdot)$ represents the first order optimality constraints associated with agent $i$ while $\rho_i^C$ and $\rho_i^I$ denote the tuning parameter vectors. Finally, $\mathbb{P}$ is the projection operator that projects $V_i$ onto its determined feasible space, denoted by $\mathcal{F}$. The feasible space is defined as the intersection of equality and inequality constraints of \eqref{generalproblem}.


Updating variables in \eqref{y_update} only involve algebraic functions. The lightweight linear structure of these federated updates is well-suited to work on resource-constrained DER controllers. This update scheme can also be implemented in a fully distributed peer-to-peer fashion or distributed with centralized oversight (i.e., where a central agent receives information update from all agents).
%The update structure accommodates both synchronous and asynchronous updates which can substantially reduce the communication overhead. Finally, the proposed method accommodates a wide-range of communication architectures. 
The updates for variables of all agents follows the following compact form:

%Consequently, the update rules for the all variables at the intra-network optimization of network $\mathcal{N}$  in a dense form is provided by (\ref{intradense})

\vspace{-.15cm}
\small
\begin{align}
\mathcal{V}(k+1)&=\widetilde{\mathcal{V}}(k)-A\widetilde{\mathcal{V}}(k)+C\nonumber\\
\widetilde{\mathcal{V}}(k+1)&=\mathbb{P} \left[ \mathcal{V}(k+1) \right]_\mathcal{F}\label{intradense}
\end{align}
\normalsize

\noindent $\mathcal{V}$ contains stacked variables for all agents, where $A$ and $C$ represent system parameters and tuning weights. Moreover, $\mathbb{P}$ is the projection operator that enforces variables to stay in the feasible space (i.e., $\mathcal{F}$). Also, $\widetilde{\mathcal{V}}$ is the vector of the stacked projected variables. Convergence analysis is presented in \cite{mohammadi2016distributed}.%the Appendix.

On a separate note, the federated computation framework being presented accommodates both synchronous and asynchronous update architectures. The difference between the two schemes is the frequency of information exchange between agents. In the synchronous update structure, every agent exchanges information with all neighboring agents after each iteration. Agents wait for each of the neighboring agents to send them updated information before performing the next update of their local variables.  Under the asynchronous update regime, some agents only exchange information after intervals of a few iterations. In this setup, agents are grouped into clusters where the exchange between agents within a cluster may take place every iteration while communication with agents in another cluster typically occurs every few iterations. These two update schemes are shown in Fig. \ref{fig:sync_async}.
Asynchronous architectures can substantially reduce the communication overhead \cite{mohammadi2015asynchronous} as inter- and intra-cluster updates follow two different clocks. 

\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{sync_async1.png}
\caption{(a) Synchronous update and (b) Asynchronous update}
\vspace{-.35cm}
\label{fig:sync_async}
\end{figure}

%{\color{red}This method also preserve privacy}

% {\color{gray}
% In this regard, Fig. 2 gives an overview of two different
% levels of distributedness. The letter B is used to indicate the
% updates of the variables at a specific bus. Fig. 2(a) shows the
% fully distributed algorithm in which computations for all buses
% are carried out at physically distinct locations, e.g., at the bus
% itself. As for each update, information only from neighboring
% buses is needed, the communication network topology is the
% same as the physical electrical system.
% In Fig. 2(b), a hybrid implementation of a distributed
% algorithm is shown. The updates for a set of buses within an
% area are carried out at a single location and communication
% takes place with neighboring areas to receive information
% about the values at the border buses over the iterations.
% Such an implementation may enable optimal coordination
% among the current control areas while achieving computational
% improvements within the control area itself.
% The question of the level of asynchronism and the level of

% distributedness may go hand-in-hand but could also be con-
% sidered separately. One can envision a completely distributed

% implementation as shown in Fig. 2(a) with either fully syn-
% chronized or with some asynchronous updates. For the hybrid

% implementation given in Fig. 2(b), while it is not necessary,
% it would be natural and probably most effective to implement
% synchronous updates within the area and asynchronous updates
% }
 



==> EE-harvesting.tex <==
%this is test

==> bibliography/output.tex <==
% Generated by IEEEtran.bst, version: 1.12 (2007/01/11)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{Delgado2018}
\BIBentryALTinterwordspacing
J.~Delgado, R.~Faria, P.~Moura, and A.~de~Almeida, ``Impacts of plug-in
  electric vehicles in the portuguese electrical grid,'' \emph{Transportation
  Research Part D: Transport and Environment}, vol.~62, pp. 372 -- 385, 2018.
  [Online]. Available: \url{https://doi.org/10.1016/j.trd.2018.03.005}
\BIBentrySTDinterwordspacing

\bibitem{RNC2050}
Portugal, ``Roadmap for carbon neutrality 2050,'' Portuguese Republic, Tech.
  Rep., 2019.

\bibitem{moura2020linking}
P.~Moura, G.~Yu, S.~Sarkar, and J.~Mohammadi, ``Linking parking and electricity
  values to unlock potentials of electric vehicles in portuguese buildings,''
  in \emph{PES General Meeting}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE,
  2020.

\bibitem{Gray2018}
\BIBentryALTinterwordspacing
M.~K. {Gray} and W.~G. {Morsi}, ``A novel transactive energy framework for
  prosumers with battery storage and electric vehicles,'' in \emph{2018 IEEE
  Electrical Power and Energy Conference (EPEC)}, Oct 2018, pp. 1--6. [Online].
  Available: \url{https://doi.org/10.1109/EPEC.2018.8598368}
\BIBentrySTDinterwordspacing

\bibitem{Liu2019b}
\BIBentryALTinterwordspacing
Z.~{Liu}, Q.~{Wu}, K.~{Ma}, M.~{Shahidehpour}, Y.~{Xue}, and S.~{Huang},
  ``Two-stage optimal scheduling of electric vehicle charging based on
  transactive control,'' \emph{IEEE Transactions on Smart Grid}, vol.~10,
  no.~3, pp. 2948--2958, May 2019. [Online]. Available:
  \url{https://doi.org/10.1109/TSG.2018.2815593}
\BIBentrySTDinterwordspacing

\bibitem{Jin2017}
\BIBentryALTinterwordspacing
X.~Jin, J.~Wu, Y.~Mu, M.~Wang, X.~Xu, and H.~Jia, ``Hierarchical microgrid
  energy management in an office building,'' \emph{Applied Energy}, vol. 208,
  pp. 480 -- 494, 2017. [Online]. Available:
  \url{https://doi.org/10.1016/j.apenergy.2017.10.002}
\BIBentrySTDinterwordspacing

\bibitem{Thomas2018}
\BIBentryALTinterwordspacing
D.~Thomas, O.~Deblecker, and C.~S. Ioakimidis, ``Optimal operation of an energy
  management system for a grid-connected smart building considering
  photovoltaics’ uncertainty and stochastic electric vehicles’ driving
  schedule,'' \emph{Applied Energy}, vol. 210, pp. 1188 -- 1206, 2018.
  [Online]. Available: \url{https://doi.org/10.1016/j.apenergy.2017.07.035}
\BIBentrySTDinterwordspacing

\bibitem{Nefedov2018}
\BIBentryALTinterwordspacing
E.~Nefedov, S.~Sierla, and V.~Vyatkin, ``Internet of energy approach for
  sustainable use of electric vehicles as energy storage of prosumer
  buildings,'' \emph{Energies}, vol.~11, no.~8, 2018. [Online]. Available:
  \url{https://doi.org/10.3390/en11082165}
\BIBentrySTDinterwordspacing

\bibitem{Quddus2018}
\BIBentryALTinterwordspacing
M.~A. Quddus, O.~Shahvari, M.~Marufuzzaman, J.~M. Usher, and R.~Jaradat, ``A
  collaborative energy sharing optimization model among electric vehicle
  charging stations, commercial buildings, and power grid,'' \emph{Applied
  Energy}, vol. 229, pp. 841 -- 857, 2018. [Online]. Available:
  \url{https://doi.org/10.1016/j.apenergy.2018.08.018}
\BIBentrySTDinterwordspacing

\bibitem{Liu2019}
\BIBentryALTinterwordspacing
Z.~{Liu}, Q.~{Wu}, M.~{Shahidehpour}, C.~{Li}, S.~{Huang}, and W.~{Wei},
  ``Transactive real-time electric vehicle charging management for commercial
  buildings with pv on-site generation,'' \emph{IEEE Transactions on Smart
  Grid}, vol.~10, no.~5, pp. 4939--4950, Sep. 2019. [Online]. Available:
  \url{https://doi.org/10.1109/TSG.2018.2871171}
\BIBentrySTDinterwordspacing

\bibitem{Fonseca2018}
\BIBentryALTinterwordspacing
P.~{Fonseca}, P.~{Moura}, H.~{Jorge}, and A.~T. {de Almeida}, ``Sustainability
  in university campus: options for achieving nearly zero energy goals,''
  vol.~19, no.~4, pp. 790--816, Jan. [Online]. Available:
  \url{https://doi.org/10.1108/IJSHE-09-2017-0145}
\BIBentrySTDinterwordspacing

\bibitem{mohammadi2019collaborative}
\BIBentryALTinterwordspacing
J.~Mohammadi and S.~Kolouri, ``Collaborative learning through shared collective
  knowledge and local expertise,'' in \emph{29th International Workshop on
  Machine Learning for Signal Processing}.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2019. [Online]. Available:
  \url{https://doi.org/10.1109/MLSP.2019.8918888}
\BIBentrySTDinterwordspacing

\end{thebibliography}


==> future-grid.tex <==
By some metrics, the electric power grid is the most complex man-made system in the world \cite{bao2009analysis}. This system spans multiple states, countries, and entire continents. Control responsibilities for this network are shared among different entities. The decision-making process occurs at different scales and across multiple spatiotemporal dimensions. The energy management paradigms of the electric grid are traditionally designed to regulate and manage a limited number of decision-making entities. Entities often control assets in a specific geographical area \cite{wood2013power}. Interactions between these entities depend on the policies and rules governing power grid operation in these areas as well as prearranged bilateral agreements. The lack of coordination to optimize cross-entity energy resources inevitably results in suboptimal system dispatch. 

% \subsection{Old grid}
% {\color{gray}
% In both cases, the task of optimally scheduling generation as well as other tasks within a control area are carried out using an Energy Management System (EMS). The coordination among neighboring control areas is generally done such that the areas agree on a flow on their tie lines and then schedule the supply of the remaining loads according to their dispatch procedure. 
% }

The future electric power grid infrastructure is emerging with a complexity that requires it be composed of many interacting elements. As the grid evolves, its new architecture should accommodate and manage an ensemble of constituent parts while ensuring interoperability and resilience. The future grid should enable plug-and-play engagement and manage heterogeneous energy resources under stress and uncertainty \cite{widergren2019grid}. The main trends behind this transition include evolving consumer expectations and technological progress. Economies of distributed electric networks are emerging at the same time, as well as growing needs for resilience given cybersecurity and environmental threats \cite{imteaj2019leveraging}.

Customers expect increased access to information and a high level of service from the twenty-first century power infrastructure. These expectations are elevated partly because outside the power sector, third party providers are offering increased choice and ease of use. For example, Uber and Lyft have disrupted the transportation system while improving it in certain respects (e.g., market-driven availability and responsiveness). On the energy side, customers demand improvements in information access as well as energy choice, equity, and reliability from their electric infrastructure. Electric grids are now expected to accommodate these rising expectations.

Technological advancements have led to ubiquitous computation and communications. This enables local information processing and decision-making and empowers customers to manage their on-site energy resources (e.g., solar PV and storage) and decide how and when to share their excess energy. Technology improvements have also unlocked new avenues for energy efficiency. For example, real-time access and coordination of building heating and cooling systems reduces their energy use and improves occupant comfort. On the other hand, the sensing and communication capabilities being added to these devices (across the spectrum of generation and consumption) creates a large attack surface for cyber intruders and can jeopardize the operations of the grid.

The energy democratization exceptions (i.e., resisting the dominant energy agenda while reclaiming and democratically restructuring energy regimes \cite{stephens2018operationalizing})  have gained steam in recent years due to access to a wider range of energy choices, widespread adoption of distributed energy resources, increased affordability of electric energy storage, and climate change considerations \cite{keshan2016}. These exceptions combined with innovative business models are encouraging local and peer-to-peer energy transactions. This shift is changing the economics of electricity generation and use.

The reliability and resilience of the aging power infrastructure is increasingly challenged by climate change, natural disasters, and cyber threats. The electric grid is key for operating other critical infrastructures.  %\cite{amini2019sustainable}. 
More specifically, any power disruption is harmful to national security, economic prosperity, and communications networks as well as the basic standard of living. The number of extreme natural weather events like wildfires, floods, storms, and heatwaves is on the rise \cite{quirin11}, \cite{yale19}. These environmental strains highlight the need for energy resiliency. For example, recent wildfires in California have pushed the state's largest utility, Pacific Gas and Electric, close to bankruptcy \cite{wsjRES}. A resilient grid is prepared to handle disruptions in the supply side caused by natural hazards, deal with cyber-physical incidents, and manage human interventions. Grid operators used to dispatch designated generation resources to preserve reliability at the time of needs. The ongoing grid transformation have enabled grid operators to access a fleet of small scale energy resources on the supply and demand sides that if orchestrated effectively can significantly boost grid resilience.
These systemic changes amplify the need for multi-entity coordination. This relies on local communication and computation capabilities. Effective coordination preserves privacy and scale across multi-modal data sources and heterogeneous devices. 



% \subsection{Transition}
% {\color{gray}
%OMPLEX SYSTEMS ARE COM- posed of many elements. Architecture concerns itself with how to manage the entire ensemble of elements that make up a system. When we think of an archi- tecture for electric power systems, the concepts need to go beyond addressing how the elements of these systems inter- operate effectively and efficiently. They must also include how they grow and evolve, how they behave under stresses and strains, and importantly, how they offer options for future decisions in an uncertain world.
% Three groups of factors are driving change to our power grids.
% ✔ Changing consumer expectations: In the era since the introduction of the smartphone, consumers expect vastly expanded choice and ease of use. These expectations have extended to energy sources. Consumers want not only to be able to choose an energy source but also to be able to easily ob- tain information related to en- ergy use.
% ✔ Emerging trends: These include technology trends, such as the availability of ubiquitous com- munications, but also demo- graphic/social trends, such as the movement toward local choice in all things, including electricity sources, as indicated by the rise of microgrids and community choice aggregators. On the negative side, the rise of cybersecurity issues that come with ubiquitous communications threatens our energy security.
% ✔ The shift from centralized elec- tricity economies of scale to distributed network economies: Twentieth century power grids were developed under the assumption that all electricity would be generated by large central-ized dispatchable generators, and these, connected via trans- mission to local distribution sys- tems, would provide a one-way flow of energy to consumers. The emergence of rooftop solar photovoltaic panels and other forms of distributed generation connected at the distribution level and the rising availability of electric energy storage are changing the economics of elec- tricity generation and use.

%Grid architecture provides a way to manage the complexity of grid modern- ization. The father of one of the coeditors once built a house (with his brothers) and later added a garage by himself. At one point, he asked his son, “When you do something like this, what do you pick up first: a shovel or a pencil?” Put that way, the answer seems obvious, but then he said, “Of course, I know some guys who try to hang the windows first.” The point here is that getting the decisions in the right order matters greatly, and grid ar- chitecture can assist in that ordering, thus avoiding the “hang the windows first” mistake and its costly consequences.
%Arguably, the most common symbol people associate with our profession is the plug, with the wall socket not far be- hind. The architectural prowess behind this simple interface powers the world. It serves to decouple the complex issues addressed by an entirely different set of electrical engineering skills that have evolved, mostly independently, over de- cades of progress on both sides of the wall. The plug and socket are presently undergoing a transformation to include the incorporation of communications. How fitting it is that our successors may see the USB port as the symbol for a new era of energy and intelligence in the modern grid. Just as most of us grew up expecting the light to go on after we plugged it in, the next generation is ex- pecting their appliances to not only “light up” but to coordinate with other equip- ment on the other side of that outlet. The tendrils of coordination go far and wide, and they deeply depend on our ability to manage the complexity using all of the architectural skills we can muster.
% }

%\subsection{The need for resilience}
%{\color{gray}
% Modern societies are heavily relying on continuous power supply provided by the electric grids. Climate change, natural disasters, and cyber threats are challenging the reliability and resilience of the aging power network. All infrastructure networks, especially urban areas are highly dependent on the electric grid power-supply [Ahmed1], [Ahmed12] and hence, the outage of such a power system can cause an enormous cost which can be considered as an utmost global concern. 
% Besides, extreme natural disasters like wildfire, hurricanes, storms, and heatwaves are just a part of the nation’s DNA and these cause power outages impacting the normal operations of companies. 

%A recent report by The Wall Street Journal claimed that one of the largest utilities of nations named PG&E is on the edge of bankruptcy because the company’s components are responsible for more than 1500 fires in recent years [Ahmed13]. Breaking out of fire one day on average, causing dozens of deaths, and responsible for the destruction of thousands of acres, the company now has the liability of more than \$30 billion according to a recent analysis. A recent survey found that power outage occurs in one in four companies at least once a month [Ahmed14]. Particularly, for large companies, power interruption loss exceeds a million dollars per hour and the annual forfeiture is around \$150 billion [Ahmed15].

% Hence, our main motivation is to mitigate such costs with the power of intelligence. We provide an outline of an adaptive resilience- based approach where the system will be resistant to power disturbance and able to cluster the risky zone from the main station. Resilience is a multidimensional attribute of a smart grid that means handling disturbances in power supply caused by natural hazards, cyber-physical incidents, or human interventions/attacks. The preeminence of resilience value in the power system with the perspective of natural disasters is one of the main goals of this paper.
% }

% \subsection{Customer perspective}
% \subsection{Grid operators perspective}
% \subsection{algorithmic view}
